Interplay Between Resilience and Accuracy in Resilient Vector Consensus in Multi-Agent Networks

In this paper, we study the relationship between resilience and accuracy in the resilient distributed multi-dimensional consensus problem. We consider a network of agents, each of which has a state in $\mathbb{R}^d$. Some agents in the network are adversarial and can change their states arbitrarily. The normal (non-adversarial) agents interact locally and update their states to achieve consensus at some point in the convex hull $\calC$ of their initial states. This objective is achievable if the number of adversaries in the neighborhood of normal agents is less than a specific value, which is a function of the local connectivity and the state dimension $d$. However, to be resilient against adversaries, especially in the case of large $d$, the desired local connectivity is large. We discuss that resilience against adversarial agents can be improved if normal agents are allowed to converge in a bounded region $\calB\supseteq\calC$, which means normal agents converge at some point close to but not necessarily inside $\calC$ in the worst case. The accuracy of resilient consensus can be measured by the Hausdorff distance between $\calB$ and $\calC$. As a result, resilience can be improved at the cost of accuracy. We propose a resilient bounded consensus algorithm that exploits the trade-off between resilience and accuracy by projecting $d$-dimensional states into lower dimensions and then solving instances of resilient consensus in lower dimensions. We analyze the algorithm, present various resilience and accuracy bounds, and also numerically evaluate our results.

==> hausdorff_distance_bound.tex <==
\section{Hausdorff Distance from box to convex hull}
Recall that Hausdorff distance from a set $A$ to a set $B$ is distance between $\sup \inf a,b$. Hausdorff distance is a standard measure of accuracy when one is interested in approximating a convex compact set in some metric space\cite{braker1998hausdorff,richardson1997approximation,schneider1988random}. 
Our consensus algorithm returns a point that is guaranteed lie in a convex region $\calB$ that we hope approximates the convex hull $\calC$ of the original pointset. Therefore, it makes sense to bound the Hausdorff distance from $\calB$ to $\calC$. If we scale a pointset, the Hausdorff distance will change with the scaling factor. To make our bound invariant to such scaling, we will instead bound the ratio of Hausdorff distance to the diameter of the pointset. Recall that the diameter of a pointset is the maximum distance between a pair of points. 

 The shape of region $\calB$, and Hausdorff distance, depends on the partition of dimension that we use to compute consensus in each part. If we partition the dimension into $d$ instances of one dimension each, this will gives an upper bound on the Hausdorff distance for all possible partitions.
\begin{fact}
Hausdorff distance from $\calB$ to $\calC$ is maximum when $\calB$ is an axis-parallel bounding box.
\end{fact}
Thus in the following our goal is to estimate the ratio of diameter and the Hausdorff distance from an axis-parallel bounding box to the convex hull. We start our discussion with the following conjecture:
\begin{conjecture}
For a given set of points in $\mathbb{R}^d$, the Hausdorff distance from the axis-parallel bounding box of the point to the convex hull of the pointset is at most $\sqrt{\frac{{d}}{2}}\times \mu(\calC)$ where $\mu(\calC)$ is the diameter of the pointset. 
\end{conjecture}
Although, we don't have a proof for the statement, we strongly believe that it is true. As an evidence, we provide proofs for the some special cases in the following. We also show that it true, the constant provided in the conjecture is best possible.

We begin by proving the conjecture in three dimensions:
%------------------------------------theorem-----------------------------------------------
\begin{theorem}
For a given set of points in $\mathbb{R}^3$, the Hausdorff distance from the axis-parallel bounding box of the pointset to the convex hull of the pointset is at most $\sqrt{ \frac{3}{2} }\times \mu(\calC)$ where $\mu(\calC)$ is the diameter of the pointset. 
\end{theorem}
%------------------------------------theorem-----------------------------------------------
%------------------------------------proof-------------------------------------------------
\textit{Proof:}\\
Without loss of generality, let all coordinates of input points be non-negative and let origin be the point on the bounding box that is at maximum distance from the convex hull. Let $a,b$ be the points of the set that lie, respectively, on faces of bounding box parallel to planes $x=0$, and $y=0$. For contradiction, assume that $\norm{a}_2,\norm{b}_2$
 is more than $\sqrt{3/2 } \mu(\calC)$. Let $\pi(a), \pi(b)$ be the respective projections of $a$, and $b$, on the plane $z=0$. Then $\norm{\pi(a)}_2^2 \ge \norm{a}_2^2 - h_z^2$, and $\norm{\pi(b)}_2^2 \ge \norm{b}_2^2 - h_z^2$, where $h_z$ is the height of the box in $z$ direction. We have,
 $$
 \begin{array}{ccc}
 \mu(\calC) &\ge& d(a,b) \ge d( \pi(a), \pi(b) ) \\
		 &=& \sqrt{ \norm{\pi(a)}_2^2 + \norm{\pi(b)}_2^2 }\\
		 &\ge&  \sqrt{ \norm{a}_2^2 - h_z^2 + \norm{b}_2^2 - h_z^2 }\\
		 &\ge&  \sqrt{ 2\frac{3}{2} \mu(\calC)^2 - 2h_z^2   }\\
 \end{array}
 $$
 We have that $2 \mu(\calC)^2 - 2h_z^2 < 0$. This is clearly a contradiction since height of a face can not be more than the diameter of the pointset. We conclude that $\min (|a|,|b|)$, and thus the Hausdorff distance from the box to the convex hull, is at most $\sqrt{ \frac{3}{2} }\times \mu(\calC)$.
 \qed
 
 \begin{figure}
\centering
\includegraphics[scale=0.5]{Thm_Proof.pdf}
\caption{Caption}
\label{fig:Thm_proof}
 \end{figure}
%---------------------------------end-proof------------------------------------------------
In the following, we show that the statement of the conjecture is true for all $d$ for certain  \textit{symmetric} pointsets. Before we state and prove the result, we need several insights into the problem.

Since translation and rotation of the points doesn't change Hausdorff distance, we may assume that the origin is a point on $\calB$ with maximum distance from $\calC$. As both $\calC$ and $\calB$ are convex, origin must be a corner vertex of the bounding box. For $\calB$ to be a minimum axis-parallel bounding box, each of the facets adjacent to origin must contain at least one point from the set $P$. 

For $1\le i\le d$, let $p_i$ be a point in $P$ closest to origin for which $i^{th}$ coordinate is zero. Then $p_1,p_2,\ldots,p_d$ define a hyperplane $X$. We observe that,
\begin{fact}
The Hausdorff distance $\delta(\calB,\calC)$ is at most Euclidean distance from origin to $X$ regardless of the positions of points $p_{d+1},p_{d+2},\ldots,p_n$.
\end{fact}
\textit{Proof:}\\
We note that the points $p_1,p_2,\ldots,p_d$ that define a hyperplane $X$ lie on the boundary of $\calB$ thus, the closest point on $X$ can't be outside the box. Also, the points in $X\cap \calB$ are a convex combination of the points $p_1,p_2,\ldots,p_d$, and must lie in their convex hull, and therefore, must also lie in the convex hull $\calC$. The claim follows.
\qed
Furthermore, 
\begin{fact}
	There exist pointset configurations for which Hausdorff distance $\delta(\calB,\calC)$ is equal to the Euclidean distance from origin to $X$. regardless of the positions of points $p_{d+1},p_{d+2},\ldots,p_n$.
\end{fact}
This clearly is the case when all of the points $p_{d+1},p_{d+2},\ldots,p_n$ lie in the halfspace defined by $X$ that does not contain origin.\\
From the previous two facts, we have that the upper bound on $\delta(\calB,\calC)$ is independent of the positions of points $p_{d+1},p_{d+2},\ldots,p_n$. Thus, we only care about the first $d$ points.
%---------------------------------theorem------------------------------------------------
 \begin{theorem}
	Let $\{p_1,p_2,\ldots,p_d \}$ be a subset of the pointset, the such that $i^{th}$ coordinate of the point $p_i$  is zero and all other coordinates are set to some constant $a$. Then, $\delta(\calB,\calC) \le (d-1)/d\sqrt{\frac{{d}}{2}}\times \mu(\calC)$.
\end{theorem}
%-------------------------------end-theorem----------------------------------------------
%----------------------------------proof----------------------------------------------
\textit{Proof:}\\
If the constant $a$ is at most $\frac{1}{ \sqrt{2} }$, then the distance of each point from the origin is bounded by $\sqrt{  \frac{d}{2}  }$ and the claim follows. Therefore, we may assume that $a > \frac{1}{ \sqrt{2} }$. We, further, assume that $d>2$.
Clearly, the diameter $\mu(\calC)$, in this case, is at least $d(p_i,p_j)$ which is given by, $\sqrt{2a^2}$. Consider the centroid point $z = \frac{1}{d}\sum_{i=1}^{d} p_i$. Then the norm of $z$ is given by,
$$
\norm{z}_2 = \sqrt{   d \left( 1/d\times (d-1)a \right)^2  }
$$

$$
\norm{z}_2 = \sqrt{d} /d\times (d-1)a 
$$


$$
\norm{z}_2 =  (d-1)/d\times \sqrt{d a^2} 
$$

We have,
$$
\norm{z}_2 =  (d-1)/d \sqrt{\frac{{d}}{2}}\times  \mu(\calC).
$$Which completes the proof. We note that as $d$ goes to infinity, $(d-1)/d$ goes to one and this ratio goes to $\sqrt{\frac{{d}}{2}}\times  \mu(\calC)$.
\qed
%-------------------------------------proof------------------------------------------------
The following proposition shows that the result in the previous theorem is best possible.
\begin{claim}
There exist point configurations for which $\delta(\calB,\calC) = (d-1)/d\sqrt{\frac{{d}}{2}}\times \mu(\calC)$.
\end{claim}
\textit{Proof:}\\
Consider a pointset that contain $2\times d$ points as follows: $\{p_1,p'_1,p_2,p'_2,\ldots,p_d,p'_d \}$, be  such that $i^{th}$ coordinate of the point $p_i$ is zero (similarly $i^{th}$ coordinate of the point $p'_i$ is one) and all other coordinates are set to some constant $1/\sqrt{2}$. Clearly, the diameter of the pointset is one in this case. The closest point to origin is the centroid $z$ of $p_1,p_2,\ldots,p_d$. We computed the norm of $z$ in the proof of previous lemma to be,
$$
\norm{z}_2 =  (d-1)/d \sqrt{\frac{{d}}{2}}\times \mu(\calC).
$$
\qed
We hope that future works can shed more light towards proving the Conjecture. We conclude this section with a following remark:
\begin{remark}
The Hausdorff distance between the convex polytope $\calB = \calC^1 \times \calC^2$ (in Algorithm \ref{algo:RBC}) and $\mathcal{C}$ is 
\begin{equation}
\label{eq:volB}
\delta(\calB,\calC) \le \max\limits_{\ell\in\{1,2\}}\mu(\calC^\ell)
\end{equation}
where $\mu(\calC^\ell)$ is the diameter of $\calC^\ell$ as defined in \eqref{eq:muCl}, and $\calC^1, \calC^2, \calC$ are covex sets in, respectively, one, two, and three dimensions.
\end{remark}
